Safety in human-multi robot collaborative scenarios: a trajectory scaling approach

In this paper, a strategy to handle the human safety in a multi-robot scenario is devised. In the presented framework, it is foreseen that robots are in charge of performing any cooperative manipulation task which is parameterized by a proper task function. The devised architecture answers to the increasing demand of strict cooperation between humans and robots, since it equips a general multi-robot cell with the feature of making robots and human working together. The human safety is properly handled by defining a safety index which depends both on the relative position and velocity of the human operator and robots. Then, the multi-robot task trajectory is properly scaled in order to ensure that the human safety never falls below a given threshold which can be set in worst conditions according to a minimum allowed distance. Simulations results are presented in order to prove the effectiveness of the approach.

==> intro.tex <==
The close cooperation of humans and robots is a highly desirable feature since it allows to benefit of the outperforming reasoning  capabilities of humans and the extreme precision and strength of robots. 
However, it is straightforward to recognize that the human safety is of the utmost importance in such a scenario that basically requires the robots to be controlled in such a way to not harm human operators~\cite{Haddadin_IJRR2009}.
The human-robot safe interaction is still an open topic and this is testified by the fact that there are not ultimate guidelines or requirements for a safe human-robot interaction and by the large effort that the scientific community has been devoting  to the matter in the last years. 
%Safety issues are investigated in the international standard ISO 10218
Initial regulations regarding human safety with respect to industrial robots can be found in the American ANSI/RIA R15.06, in the European EN 775 or in the more general international standard ISO 10218 and the technical specification document ISO/TS 15066. %{\red non saprei se vanno citati o va bene solo il nome dello std}
In detail, the latter exactly focuses on human-robot collaborative scenarios and   envisages four possible safe interactions: 
\begin{enumerate}
\item safety-rated monitored stop, i.e. robots are required to stop when humans enter the working area;
\item hand guiding, i.e. robots are required to follow human manual guidance;
\item \label{en:iso_ssm} speed and separation monitoring, i.e. robots are required to keep a minimum safety distance from operators;
\item \label{en:iso_pfl} power and force limiting, i.e. robots are required to mitigate human harm in the case of impact.  
\end{enumerate}
%the technical specification includes quantitative biomechanical limits, such as allowable peak forces or pressures for various parts of the body, as well as equations for speed and separation monitoring
It is clear that interactions~\ref{en:iso_ssm} and \ref{en:iso_pfl} involve integrating the robot autonomous task with human safety requirements. Therefore,  if on the one hand breaking the division barriers between humans and robots in industrial environments drastically increases their flexibility, on the other hand it opens several challenges in terms of real-time planning capabilities as well as of technologies to enable robots gain awareness of their surroundings.
%to empower robots to become aware of their surroundings; 
 In particular, as highlighted in~\cite{Gomez_IEEAccess2017}, different sensor features may be required depending on the nature of the interaction: from  sensors for detecting operators sharing the same working area in the case of collision prevention, e.g. motion capture systems, range sensors or artificial vision systems as in~\cite{Flacco_ICRA2012}, to sensors for assessing force exchange when an impact occurs in the case of power and force limiting interaction, e.g. force or tactile sensors as in~\cite{Cirillo_RAL2016}. 
% In the case of collision prevention, adequate exteroceptive sensors are necessary to detect operators in the shared environment, thus allowing avoidance strategies to be undertaken, e.g. artificial vision systems, motion capture systems or range sensors. The work in~\cite{Flacco_ICRA2012} proposes...
% %via suitable avoidance strategies or minimization of human injuries in the case of impacts for which suitable metrics to assess induced damage are proposed in..  
%In the case of minimization of human injuries during impact, mechanical compliance systems integrated in industrial robot are typically involved or  lightweight robots are adopted whose reduced inertia implies a reduced possible damage; moreover, robots can be equipped with tactile or force sensors in order to detect collision events and engage proper control strategies. 
Although power and force limiting is crucial in the case of physical human-robot interaction where contact is unavoidable, distance monitoring would be more suitable for pure coexistence in the working area. 
%In this work, we are interested in exploring real-time strategies for the latter typology of interaction, i.e. for collision prevention in shared environments without dealing with perception problems. 
In the latter scenario, it becomes relevant to quantify the level of human safety, looking at the overall structure of the manipulator as a source of danger to humans, so that the robots behaviour can be adapted accordingly. %{\red to add: indice che non tiene conto della struttura, quindi dire che kulic e zanchettin si}
An index based on distance, velocity and inertial contributions is proposed in~\cite{Kulic_RAS2006} and is evaluated for the nearest point between each link and the operator; then, such danger index is exploited to generate a virtual repulsive force according to artificial  potential field theory in~\cite{Khatib_ICRA1985}. The study presented in~\cite{Zanchettin_TRO2013} also focuses on defining an assessment of human safety which is now based on velocity and distance terms and is extended to the overall structure of the manipulator by a proper integration along each link; a gradient-based technique is then adopted to drive the manipulator. 
The previous approaches rely on pursuing evasive actions to increase safety, however, in industrial setting, it is generally recommended to follow the desired task path without deviating from it. 
% by changing the desired path for the robot task, however, in industrial environments this may not be advisable.
This guideline is broadened in~\cite{Zanchettin_TASE2016} where robot velocity is modulated in accordance with the distance from the operator while preserving the nominal task path. A further approach is presented in~\cite{Liu_ICRA2016} and~\cite{Kimmel_TRO2017} where the safe interaction problem is modeled as an invariance control problem, i.e. it is based on defining a safe set of robot states for which no collision with humans occurs and then on making this set invariant.
\\Finally, other solutions exploit the prediction of human motion in order to obtain proactive strategies rather than to frequently re-plan the trajectory. %As an example, the work in~\cite{Perez_ICRA2015} ...
%The major drawback in prediction-based strategies is that human behaviour is extremely variable and unpredictable and, in turn, adapts to robot behaviour; thus 
However, in order to face the extreme variability and unpredictability of human behaviours, only a subset of possible human actions is generally supported and predicted, as reaching motions in~\cite{Perez_ICRA2015} or repetitive actions in~\cite{Wang_RAL2018}.
\\The previous works testify to the fervour in research regarding human-robot interaction and, consequently, human safety; however, to the authors' knowledge, the case of coexistence with multi-manipulators systems has not yet been investigated. In this context, human safety must certainly remain the highest priority task, but at the same time the coordination of the robot team must be managed.
%this means that the avoidance strategy can not act independently on each single robot whereas it must adequately modify the global cooperative task taking into account any constraints introduced by it, e.g. the case of tightly connected robots. 
%Finally, it is worth reminding that human-robot collaboration and decentralized control architectures are both key points behind the strategic initiative of {\it Industry 4.0} and {\it Factories of the Future Roadmap 2020}. 
\\Motivated by these considerations, this study  presents a general solution for handling the human safety in a multi-robot scenario where robots are assigned to accomplish a cooperative task which is properly parameterized by task functions. Starting from the definition of a  safety index depending on the human operator's state and on the state of a generic point of the robot structure, first the safety associated to the whole robot and, then, to whole team are computed.
This safety measure is properly adopted to  modify the robot trajectories in order to preserve the cooperative task and so as to not violate the safety requirements. However, because of the constraint represented by the task itself this might result in a too restrictive strategy that might lead to the violation of the established requirements. When this case occurs, the task is interrupted and an impedance-based strategy is adopted; task is finally recovered when the safety conditions are restored.\\
The devised solution presents several desirable features with respect to other solutions cited above:
\begin{itemize}
\item it works for general expressions of the safety index; 
\item it explicitly takes into account the multi-robot nature of the task;
\item it does not modify the task path or require the task to be aborted unless if necessary.
\end{itemize}
The paper is organized as follows.
Section~\ref{sec:mathbackground} introduces the mathematical background and the problem setting.
In Section~\ref{sec:humansafetyassess}, the adopted safety index is defined and analyzed in detail, while in Section~\ref{sec:humanavoidance} this index is exploited to define a  safe human-robot interaction strategy.
Finally, numerical simulations and conclusions are presented in Sections~\ref{sec:case_study} and \ref{sec:conclusions}, respectively.

%{\red da qui è  med\\
% In~\cite{Marvel_TASE2013}, two main approaches to guarantee the human safety  are identified, namely, the power and force limiting and the speed and position monitoring. The former aims at limiting the human injury in the case of impact with a robot and is exploited, for example,  in~\cite{Bicchi_RAM2004} to design a variable compliance at actuation level, and in~\cite{Haddadin_IROS2008}, that introduces different  collision detection and reaction techniques based on the reduction of contact forces. 
%On the contrary, the latter aims at avoiding any possible collision by keeping a certain safety distance between robots and operators. To the purpose, it is necessary to develop real-time motion planning capabilities that enable the distance constraint to be satisfied in accordance with the dynamic behaviour of human operators. 
%%In order to guarantee the distance constraints, it becomes necessary to develop real-time motion planning capabilities that enable to take into account the dynamic behaviour of human operators. 
%While a force limiting strategy is a key feature for physical human-robot interaction and collaborative tasks, an avoidance strategy may be more appropriate in the case of space sharing without explicit human-robot collaboration. 
%\\The most common avoidance approach is based on the theory of artificial potential field~\cite{Khatib_ICRA1985}, according to which the robot motion is guided by attractive forces towards the desired configuration and repulsive ones that move it away from obstacles. 
%The reactive collision avoidance strategy presented in~\cite{Haddadin_IROS2010} exploits this principle and  reacts if virtual or physical contact occurs with the robot.\\
%%A general drawback of this method is that it does not capture the relative motion between robot and obstacles.
%%This approach is exploited by~\cite{Flacco_ICRA2012} where the repulsive force considers both positions and velocities of obstacles. Moreover, multiple control points on both manipulator structure and surfaces of obstacles are taken into account. 
%%Other metrics to generate repulsive contributions can be found in~\cite{Zanchettin_TRO2013} and \cite{Kulic_RAS2006}.  
%%Concerning Other metrics to generate repulsive contributions can be found in~\cite{Zanchettin_TRO2013} and \cite{Kulic_RAS2006}.  
%%kulic: path planning according to the minimization of a danger function
%%Further solutions for human avoidance take advantage of the prediction of the movement of human operators to achieve a more proactive behaviour towards them~\cite{Wang_RAL2018} is based on such a prediction to solve a constrained optimization problem aimed at ensuring a minimum safety distance during the prediction time window. However, the adopted prediction technique is only suitable if the operator performs repetitive actions. 
%%In~\cite{Tamura_IJARS2013}, the authors classify pedestrian behaviours into a finite number of defined patterns according to which the motion prediction varies; thus, once the current pattern of the person has been estimated, the robot trajectory is modulated taking into account the reliability of the prediction. 
%The work in \cite{Zanchettin_TRO2013} defines a quantity, named danger field, that quantifies  how dangerous the robot state is to the objects or people in the environment.  This information is then used  in order to make the motion of the robot safer to the environment by modifying the robot path.
%%\\ A further approach to ensuring safety is to scale the nominal trajectory in speed as a function of the human safety level. Although trajectory scaling is a well-known problem in robot trajectory planning to meet kinematic and dynamic constraints, it is not particularly widespread for human safety issues {\red citare cosa?}.  
%Since in industrial environments the deviation from the nominal path may not be acceptable or at least not desirable, a possible solution can be to scale only the speed of the nominal trajectory, preserving its path, in case the safety of objects or people is compromised. This approach is explored in~\cite{Zanchettin_TASE2016} where human safety is assessed by a metrics based on robot braking time and is handled as a hard constraint in a Linear Programming optimization problem that aims to maximize scaling factor  while meeting kinematic and safety constraints.
%}
